Asymmetry in Polymer-Solvent Interactions Yields Complex Thermoresponsive Behavior

Thermoresponsive polymers hold both fundamental and technological importance, but the essential physics driving their intriguing behavior is not wholly understood. We introduce a lattice framework that incorporates elements of Flory-Huggins solution theory and the $q$-state Potts model to study the phase behavior of polymer solutions and single-chain conformational characteristics. Importantly, the framework does not employ any temperature- or composition-dependent parameters. With this minimal Flory-Huggins-Potts framework, we show that orientation-dependent interactions, specifically between monomer segments and solvent particles, are alone sufficient to observe upper critical solution temperatures, miscibility loops, and hourglass-shaped spinodal curves. Signatures of emergent phase behavior are found in single-chain Monte Carlo simulations, which display heating- and cooling-induced coil-globule transitions linked to energy fluctuations. The model also capably describes a range of experimental systems. This work provides new insights regarding the microscopic physics that underpin complex thermoresponsive behavior in polymers.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
